Reactive Global Minimum Variance Portfolios with $k-$BAHC covariance cleaning

We introduce a $k$-fold boosted version of our Boostrapped Average Hierarchical Clustering cleaning procedure for correlation and covariance matrices. We then apply this method to global minimum variance portfolios for various values of $k$ and compare their performance with other state-of-the-art methods. Generally, we find that our method yields better Sharpe ratios after transaction costs than competing filtering methods, despite requiring a larger turnover.

==> TABLE/Gross_longshort_False.tex <==
\begin{tabular}{lcccccccccc}
\toprule
& \multicolumn{2}{l}{Covariance matrix estimators } \\ \cmidrule{2-11}
$\tau_{in}$&  Sample &   CV &  $1-$BAHC &  $2-$BAHC &  $3-$BAHC &  $4-$BAHC &  $7-$BAHC &  $11-$BAHC &  $18-$BAHC &  $30-$BAHC \\\midrule
21   &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
42   &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
63   &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
84   &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
105  &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
126  &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
147  &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
168  &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
189  &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
210  &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
231  &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
252  &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
\midrule 
300  &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
350  &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
400  &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
500  &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
750  &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
1000 &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
1500 &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
2000 &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\\bottomrule
\end{tabular}


==> TABLE/N90_longshort_False.tex <==
\begin{tabular}{lcccccccccc}
\toprule
& \multicolumn{2}{l}{Covariance matrix estimators } \\ \cmidrule{2-11}
$\tau_{in}$&  Sample &  CV &  $1-$BAHC &  $2-$BAHC &  $3-$BAHC &  $4-$BAHC &  $7-$BAHC &  $11-$BAHC &  $18-$BAHC &  $30-$BAHC \\\midrule
21   &     279 & 179 &\textbf{15}&        24 &        33 &        38 &        50 &         58 &         65 &         69  \\
42   &      30 & 103 &\textbf{14}&        20 &        24 &        28 &        35 &         40 &         44 &         46  \\
63   &      20 &  82 &\textbf{15}&        19 &        23 &        26 &        31 &         35 &         38 &         39  \\
84   &      19 &  71 &\textbf{15}&        19 &        22 &        24 &        28 &         31 &         34 &         35  \\
105  &      19 &  63 &\textbf{16}&        19 &        21 &        23 &        27 &         30 &         32 &         33  \\
126  &      19 &  60 &\textbf{16}&        19 &        21 &        23 &        26 &         28 &         30 &         31  \\
147  &      20 &  56 &\textbf{16}&        19 &        21 &        23 &        25 &         27 &         29 &         30  \\
168  &      20 &  54 &\textbf{17}&        19 &        21 &        22 &        25 &         27 &         28 &         29  \\
189  &      20 &  52 &\textbf{17}&        19 &        21 &        22 &        24 &         26 &         27 &         28  \\
210  &      20 &  50 &\textbf{17}&        19 &        21 &        22 &        24 &         25 &         27 &         27  \\
231  &      20 &  49 &\textbf{17}&        19 &        21 &        22 &        24 &         25 &         26 &         27  \\
252  &      20 &  48 &\textbf{17}&        19 &        21 &        22 &        23 &         25 &         26 &         26  \\
\midrule 
300  &      20 &  46 &\textbf{18}&        19 &        20 &        21 &        23 &         24 &         25 &         25  \\
350  &      20 &  44 &\textbf{18}&        19 &        20 &        21 &        22 &         23 &         24 &         25  \\
400  &      20 &  42 &\textbf{18}&        19 &        20 &        21 &        22 &         23 &         24 &         24  \\
500  &      20 &  40 &\textbf{18}&        19 &        20 &        21 &        21 &         22 &         22 &         23  \\
750  &      20 &  36 &\textbf{18}&\textbf{18}&        19 &        19 &        20 &         20 &         21 &         21  \\
1000 &      20 &  33 &\textbf{17}&        18 &        18 &        19 &        19 &         20 &         20 &         21  \\
1500 &      20 &  29 &\textbf{18}&\textbf{18}&\textbf{18}&        19 &        19 &         19 &         20 &         20  \\
2000 &      19 &  26 &\textbf{17}&        18 &        18 &        18 &        18 &         19 &         19 &         19  \\\bottomrule
\end{tabular}


==> TABLE/Neff_longshort_True.tex <==
\begin{tabular}{lcccccccccc}
\toprule
& \multicolumn{2}{l}{Covariance matrix estimators } \\ \cmidrule{2-11}
$\tau_{in}$&  Sample &    CV &  $1-$BAHC &  $2-$BAHC &  $3-$BAHC &  $4-$BAHC &  $7-$BAHC &  $11-$BAHC &  $18-$BAHC &  $30-$BAHC \\\midrule
21   &   254.9 & 230.0 &\textbf{33.4}&      34.0 &      36.8 &      39.1 &      44.3 &       48.5 &       52.4 &       55.3  \\
42   &   153.5 & 154.1 &      31.3 &\textbf{29.8}&      31.5 &      33.1 &      36.5 &       39.2 &       41.8 &       43.6  \\
63   &   107.0 & 123.3 &      30.4 &\textbf{27.8}&      28.9 &      30.1 &      32.6 &       34.6 &       36.4 &       37.5  \\
84   &    82.0 & 105.6 &      29.8 &\textbf{26.5}&      27.3 &      28.1 &      30.1 &       31.6 &       33.0 &       33.7  \\
105  &    66.0 &  91.3 &      29.6 &\textbf{25.6}&      26.1 &      26.8 &      28.5 &       29.8 &       30.8 &       31.3  \\
126  &    54.7 &  84.8 &      29.4 &\textbf{25.0}&      25.4 &      26.0 &      27.3 &       28.4 &       29.3 &       29.5  \\
147  &    46.2 &  77.9 &      29.3 &\textbf{24.5}&      24.6 &      25.1 &      26.3 &       27.3 &       27.9 &       28.0  \\
168  &    39.6 &  72.6 &      29.2 &\textbf{24.0}&\textbf{24.0}&      24.4 &      25.4 &       26.3 &       26.8 &       26.8  \\
189  &    34.4 &  68.1 &      29.1 &      23.6 &\textbf{23.3}&      23.6 &      24.5 &       25.2 &       25.7 &       25.6  \\
210  &    29.9 &  64.0 &      28.9 &      23.2 &\textbf{22.7}&      23.0 &      23.8 &       24.4 &       24.8 &       24.7  \\
231  &    26.2 &  61.0 &      28.8 &      22.9 &\textbf{22.3}&      22.5 &      23.2 &       23.8 &       24.1 &       23.9  \\
252  &    23.0 &  58.2 &      28.6 &      22.5 &\textbf{21.8}&      21.9 &      22.6 &       23.1 &       23.4 &       23.1  \\
\midrule 
300  &\textbf{0.1}&  52.4 &      28.0 &      21.6 &      20.7 &      20.8 &      21.2 &       21.6 &       21.8 &       21.6  \\
350  &\textbf{0.1}&  48.0 &      27.5 &      20.9 &      19.8 &      19.8 &      20.2 &       20.5 &       20.7 &       20.3  \\
400  &\textbf{0.0}&  44.4 &      27.0 &      20.2 &      19.0 &      18.9 &      19.2 &       19.5 &       19.6 &       19.3  \\
500  &\textbf{0.4}&  38.9 &      26.0 &      19.1 &      17.6 &      17.5 &      17.7 &       17.9 &       17.9 &       17.5  \\
750  &\textbf{2.3}&  30.5 &      24.2 &      17.2 &      15.5 &      15.2 &      15.2 &       15.3 &       15.3 &       14.9  \\
1000 &\textbf{4.6}&  25.6 &      22.4 &      15.6 &      14.1 &      13.8 &      13.7 &       13.7 &       13.7 &       13.4  \\
1500 &\textbf{7.3}&  20.2 &      19.5 &      13.6 &      12.5 &      12.2 &      12.0 &       12.0 &       11.9 &       11.6  \\
2000 &\textbf{8.4}&  17.1 &      17.1 &      12.3 &      11.6 &      11.2 &      11.0 &       10.9 &       10.8 &       10.6  \\\bottomrule
\end{tabular}


==> TABLE/SR_longshort_False.tex <==
\begin{tabular}{lccccccccccc}
\toprule
& \multicolumn{2}{l}{Covariance matrix estimators } \\ \cmidrule{2-12}
$\tau_{in}$&   EQ &  Sample &   CV &  $1-$BAHC &  $2-$BAHC &  $3-$BAHC &  $4-$BAHC &  $7-$BAHC &  $11-$BAHC &  $18-$BAHC &  $30-$BAHC \\\midrule
21   & 0.53 &    0.45 & 0.61 &      0.60 &      0.61 &      0.62 &      0.63 &      0.64 &       0.64 &\textbf{0.65}&\textbf{0.65} \\
42   & 0.52 &    0.73 & 0.68 &      0.67 &      0.71 &      0.74 &      0.75 &\textbf{0.78}&\textbf{0.78}&\textbf{0.78}&       0.77  \\
63   & 0.51 &    0.89 & 0.79 &      0.89 &      0.91 &      0.93 &      0.94 &      0.97 &\textbf{0.98}&\textbf{0.98}&\textbf{0.98} \\
84   & 0.51 &\textbf{0.95}& 0.79 &      0.87 &      0.88 &      0.89 &      0.91 &      0.92 &       0.92 &       0.92 &       0.92  \\
105  & 0.50 &    0.85 & 0.81 &      0.83 &      0.84 &      0.87 &      0.89 &      0.91 &       0.92 &\textbf{0.93}&       0.92  \\
126  & 0.50 &    0.95 & 0.89 &      0.91 &      0.93 &      0.96 &      0.97 &      0.99 &\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
147  & 0.50 &    0.94 & 0.85 &      0.90 &      0.91 &      0.93 &      0.94 &      0.95 &       0.96 &\textbf{0.97}&\textbf{0.97} \\
168  & 0.49 &    0.89 & 0.84 &      0.91 &      0.92 &      0.93 &      0.94 &      0.94 &\textbf{0.95}&       0.94 &       0.94  \\
189  & 0.49 &    0.96 & 0.86 &      0.96 &\textbf{0.98}&      0.97 &\textbf{0.98}&\textbf{0.98}&\textbf{0.98}&\textbf{0.98}&\textbf{0.98} \\
210  & 0.49 &    0.94 & 0.84 &\textbf{0.98}&      0.96 &      0.96 &      0.96 &      0.96 &       0.96 &       0.96 &       0.95  \\
231  & 0.48 &    0.85 & 0.81 &\textbf{0.88}&      0.87 &      0.86 &      0.86 &      0.85 &       0.85 &       0.84 &       0.84  \\
252  & 0.48 &    0.80 & 0.78 &\textbf{0.86}&      0.83 &      0.83 &      0.82 &      0.82 &       0.82 &       0.81 &       0.81  \\
\midrule 
300  & 0.47 &    0.79 & 0.79 &\textbf{0.84}&      0.81 &      0.81 &      0.81 &      0.82 &       0.82 &       0.82 &       0.82  \\
350  & 0.47 &    0.88 & 0.83 &\textbf{0.90}&      0.88 &      0.86 &      0.87 &      0.88 &       0.88 &       0.88 &       0.88  \\
400  & 0.47 &    0.90 & 0.82 &\textbf{0.92}&      0.90 &      0.88 &      0.87 &      0.88 &       0.88 &       0.88 &       0.89  \\
500  & 0.46 &    0.82 & 0.81 &\textbf{0.87}&      0.84 &      0.83 &      0.83 &      0.83 &       0.83 &       0.83 &       0.82  \\
750  & 0.45 &    0.79 & 0.80 &\textbf{0.85}&      0.83 &      0.81 &      0.79 &      0.78 &       0.78 &       0.78 &       0.78  \\
1000 & 0.44 &    0.80 & 0.82 &\textbf{0.86}&      0.83 &      0.82 &      0.81 &      0.81 &       0.81 &       0.81 &       0.81  \\
1500 & 0.42 &    0.81 & 0.82 &\textbf{0.86}&      0.85 &      0.84 &      0.83 &      0.82 &       0.82 &       0.82 &       0.82  \\
2000 & 0.39 &    0.78 & 0.76 &      0.78 &\textbf{0.80}&\textbf{0.80}&      0.79 &      0.79 &       0.79 &       0.79 &       0.79  \\\bottomrule
\end{tabular}


==> TABLE/SR_longshort_True.tex <==
\begin{tabular}{lccccccccccc}
\toprule
& \multicolumn{2}{l}{Covariance matrix estimators } \\ \cmidrule{2-12}
$\tau_{in}$&   EQ &  Sample &   CV &  $1-$BAHC &  $2-$BAHC &  $3-$BAHC &  $4-$BAHC &  $7-$BAHC &  $11-$BAHC &  $18-$BAHC &  $30-$BAHC \\\midrule
21   & 0.53 &     NaN & 0.65 &      0.60 &      0.62 &      0.64 &      0.65 &      0.67 &       0.68 &\textbf{0.69}&\textbf{0.69} \\
42   & 0.52 &     NaN & 0.67 &      0.61 &      0.66 &      0.69 &      0.71 &      0.74 &       0.75 &       0.75 &\textbf{0.76} \\
63   & 0.51 &    0.67 & 0.80 &      0.84 &      0.91 &      0.97 &      1.00 &      1.03 &\textbf{1.04}&\textbf{1.04}&       1.03  \\
84   & 0.51 &    0.65 & 0.84 &      0.86 &      0.96 &      1.00 &      1.03 &      1.08 &\textbf{1.09}&       1.08 &       1.07  \\
105  & 0.50 &    0.64 & 0.87 &      0.88 &      0.98 &      1.04 &      1.05 &      1.09 &\textbf{1.10}&\textbf{1.10}&       1.09  \\
126  & 0.50 &    0.71 & 0.87 &      0.83 &      0.92 &      0.95 &      0.96 &      1.01 &\textbf{1.02}&\textbf{1.02}&       1.01  \\
147  & 0.50 &    0.74 & 0.88 &      0.80 &      0.89 &      0.94 &      0.98 &      1.05 &\textbf{1.06}&\textbf{1.06}&       1.05  \\
168  & 0.49 &    0.73 & 0.87 &      0.78 &      0.87 &      0.91 &      0.94 &      0.98 &\textbf{1.00}&\textbf{1.00}&\textbf{1.00} \\
189  & 0.49 &    0.68 & 0.90 &      0.78 &      0.90 &      0.92 &      0.95 &      0.99 &       1.03 &       1.04 &\textbf{1.05} \\
210  & 0.49 &    0.68 & 0.88 &      0.81 &      0.92 &      0.96 &      0.99 &      1.02 &       1.03 &\textbf{1.04}&\textbf{1.04} \\
231  & 0.48 &    0.60 & 0.91 &      0.74 &      0.85 &      0.90 &      0.91 &      0.93 &\textbf{0.94}&\textbf{0.94}&\textbf{0.94} \\
252  & 0.48 &    0.51 & 0.89 &      0.73 &      0.83 &      0.85 &      0.86 &      0.89 &       0.92 &\textbf{0.93}&\textbf{0.93} \\
\midrule 
300  & 0.47 &     NaN &\textbf{1.00}&      0.75 &      0.87 &      0.90 &      0.92 &      0.95 &       0.95 &       0.97 &       0.97  \\
350  & 0.47 &     NaN & 1.00 &      0.79 &      0.87 &      0.89 &      0.92 &      0.97 &       0.99 &       0.99 &\textbf{1.01} \\
400  & 0.47 &     NaN &\textbf{1.03}&      0.79 &      0.88 &      0.92 &      0.95 &      0.98 &       0.99 &       0.99 &       0.98  \\
500  & 0.46 &     NaN & 0.99 &      0.76 &      0.90 &      0.93 &      0.95 &      0.98 &       0.99 &\textbf{1.00}&       0.99  \\
750  & 0.45 &     NaN & 0.94 &      0.79 &      0.91 &      0.94 &\textbf{0.95}&      0.94 &       0.94 &       0.92 &       0.90  \\
1000 & 0.44 &    0.13 & 0.92 &      0.80 &      0.87 &      0.94 &      0.97 &\textbf{1.03}&       1.02 &       1.00 &       0.96  \\
1500 & 0.42 &    0.93 & 1.08 &      0.83 &      0.97 &      1.04 &      1.08 &\textbf{1.12}&\textbf{1.12}&       1.11 &       1.11  \\
2000 & 0.39 &    0.96 &\textbf{0.99}&      0.81 &      0.90 &      0.89 &      0.90 &      0.94 &       0.96 &       0.98 &\textbf{0.99} \\\bottomrule
\end{tabular}

